BPS States in the Duality Web of the Omega deformation

In this note, we study different limits of an Omega-deformed (2,0) six-dimensional gauge theory realized in a M-theory fluxtrap background. Via a chain of dualities, we connect the Omega-deformed SYM to a new four-dimensional gauge theory which we refer to as the reciprocal gauge theory. This theory has several properties in common with Liouville field theory, such as its gauge coupling b^2 =\epsilon_2 / \epsilon_1, and its behavior under S-duality. Finally, we realize the BPS states on the SYM side of the AGT correspondence and follow them along the chain of dualities. In the fluxtrap frame, we are dealing with two distinct types of states localized in different radial positions, while in the reciprocal frame, we find single states carrying both charges localized in one place which appear to be perturbatively stable. Our microscopic picture of the small-b limit exhibits semiclassically BPS bound states, which are not visible at the level of the partition function.

==> pollo <==
\NeedsTeXFormat{LaTeX2e}[1999/12/01]
\ProvidesPackage{Packages}


%
%
%
%
%

\RequirePackage[pdftex,final]{graphicx}
\graphicspath{{Plots/}}

\RequirePackage{mathtools}

\newif{\if@Packages@showonlyrefs}
\@Packages@showonlyrefsfalse

\DeclareOption{showonlyrefs}{\@Packages@showonlyrefstrue}


\ProcessOptions

\if@Packages@showonlyrefs
  \mathtoolsset{showonlyrefs,showmanualtags}
\fi


%
\newcommand{\preprint}[1]{%
  \RequirePackage{fancyhdr}
  \fancypagestyle{empty}{%
    \fancyhf{} %
    \fancyhead[R]{{#1}}
    \renewcommand{\headrulewidth}{0pt} 
    \renewcommand{\footrulewidth}{0pt}
  }
}

\frenchspacing

\RequirePackage[margin=10pt,font=small,labelfont=bf,width=14cm]{caption}
%

\RequirePackage{tikz} 
\usetikzlibrary{shapes.arrows}
\RequirePackage{booktabs}

%
%
\RequirePackage{array}
\RequirePackage{multirow}
\RequirePackage{colortbl}

\RequirePackage{nicefrac}
\RequirePackage[]{xcolor}

%
\RequirePackage{amsmath,amssymb,amsxtra}

%
\RequirePackage[T1]{fontenc}
\RequirePackage[utf8]{inputenc}

%
\RequirePackage{mathrsfs}
%
\RequirePackage[scaled]{berasans}
\RequirePackage[sc,osf]{mathpazo}

\RequirePackage{microtype}

%
\RequirePackage{sectsty}
\allsectionsfont{\sffamily}
\renewcommand*{\abstractname}{\sffamily Abstract}

\RequirePackage{wasysym}
\RequirePackage{bbm}



%

%
\RequirePackage{setspace}
\RequirePackage{xspace}
%
%
%
%
%
%
%
%
%
%


%
\RequirePackage{braket}

%
\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
%
,linktocpage=true
]{hyperref}

%

%
%
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{%
  \printtext{\bibstring{in}\intitlepunct}}}

%
\DeclareFieldFormat[article]{title}{\mkbibemph{#1}} 

%
\setlength{\bibitemsep}{0.3\baselineskip}

%
\renewcommand{\bibfont}{\normalfont\small}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%

\RequirePackage{tensor}
\RequirePackage{slashed}

\RequirePackage{acronym}

\RequirePackage[ragged,marginal]{footmisc}

%
\RequirePackage[a4paper,top=3cm,bottom=3cm]{geometry}
%

%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%

%
%
%
%
%
%

%
%
%
%
%

%
%

%
%
%
%

%
%
%
%
%
%
%
%


\endinput

